The Competition Complexity of Auctions: A Bulow-Klemperer Result for Multi-Dimensional Bidders

A seminal result of Bulow and Klemperer [1989] demonstrates the power of competition for extracting revenue: when selling a single item to $n$ bidders whose values are drawn i.i.d. from a regular distribution, the simple welfare-maximizing VCG mechanism (in this case, a second price-auction) with one additional bidder extracts at least as much revenue in expectation as the optimal mechanism. The beauty of this theorem stems from the fact that VCG is a {\em prior-independent} mechanism, where the seller possesses no information about the distribution, and yet, by recruiting one additional bidder it performs better than any prior-dependent mechanism tailored exactly to the distribution at hand (without the additional bidder). In this work, we establish the first {\em full Bulow-Klemperer} results in {\em multi-dimensional} environments, proving that by recruiting additional bidders, the revenue of the VCG mechanism surpasses that of the optimal (possibly randomized, Bayesian incentive compatible) mechanism. For a given environment with i.i.d. bidders, we term the number of additional bidders needed to achieve this guarantee the environment's {\em competition complexity}. Using the recent duality-based framework of Cai et al. [2016] for reasoning about optimal revenue, we show that the competition complexity of $n$ bidders with additive valuations over $m$ independent, regular items is at most $n+2m-2$ and at least $\log(m)$. We extend our results to bidders with additive valuations subject to downward-closed constraints, showing that these significantly more general valuations increase the competition complexity by at most an additive $m-1$ factor. We further improve this bound for the special case of matroid constraints, and provide additional extensions as well.

==> benchmark_fail_example.tex <==


We now present an example where the previous benchmark used in \cite{CDW16} fails to provide any meaningful bounds on the competition complexity. In our example, the original market has a single bidder and only two items. Item $a$ is distributed according to the equal revenue distribution capped at some value $k$; \textit{i.e.}, $$F_a(x)=\begin{cases}
1-1/x \quad & x < k\\
1 \quad & x=k
\end{cases},$$
supported on $[1,k]$.
Item $b$ is distributed according to the following CDF: $F_b(x)=\frac{k+1}{k}\left(1-\frac{1}{x-k+1}\right),$ supported on $[k,2k]$. One can verify that both distributions are regular. 
Consider the benchmark \eqref{eq:bench0} proposed by \cite{CDW16}, which in the case of two items is interpreted as the expected virtual value of the item with the highest value of the two \textit{plus} the expected value of the item with the lower value of the two. Since item $b$ always has a higher value than item $a$, this is exactly the expected virtual value of item $b$ \textit{plus} the expected value of item $a$. The expected value of item $a$ is 
\begin{eqnarray*}
	\int_{0}^{k}(1-F(x)) dx + k\cdot \frac{1}{k} = 1 + \int_{1}^{k}\frac{1}{x} dx + 1 = 2+\ln k.
\end{eqnarray*}
As for the expected virtual value of item $b$, consider the virtual valuation function of item $b$,	$\varphi_b(x)=x-\frac{1-F_b(x)}{f_b(x)}$.
since $F_b$ is regular, the virtual value is monotone non-decreasing, and therefore gets the minimal value for $x=k$. Therefore, the expected virtual value of item $b$ is at least the minimal virtual value $$\varphi_b(k)=k-\frac{1}{f_b(k)}=k-\frac{1}{\frac{k+1}{k}\cdot \frac{1}{\left(k-k+1\right)^2}}= k-\frac{k}{k+1}\geq k-1.$$

Combining the expected value of item $a$ and the lower bound on the expected virtual value of item $b$, we get that the benchmark is at least $2+\ln k + k - 1 = k+\ln k + 1$.

Now consider running $\VCG$ using $\ell$ bidders in total ($\ell-1$ additional bidders). Since running $\VCG$ with additive bidders is the same as running $\VCG$ for each item separately, we analyze how much revenue we get by running $\VCG$ for each item. We first analyze the revenue from running Myerson's optimal mechanism on item $a$ with $\ell$ bidders (which is an upper bound on running $\VCG$). The expected revenue of the optimal single-bidder auction is $1$.
By revenue submodularity (\cite{DughmiRS12}), the expected revenue of running the optimal mechanism is a concave function of the number of bidders. Thus, the expected revenue of the optimal auction with $\ell$ bidders is at most $\ell$.


\begin{figure}[H]
	\centering
	\begin{tikzpicture}[framed]
	\begin{axis}[
	axis lines = left,
	xlabel = $q$,
	ylabel = {$R(q)$},
	xtick = {0,1},
	ytick = {0,1,10},
	yticklabels = {$0$,$1$,$k$},
	ymin = 0,
	legend pos=north west]
	]
	%Below the red parabola is defined
	\addplot [
	domain=0:1, 
	samples=100, 
	color=red,
	very thick
	]
	{1+(10-1)*x};
	\addlegendentry{$G_b$}
	
	\addplot [
	domain=0:1, 
	samples=100, 
	color=blue,
	very thick,
	densely dotted
	]
	{x*(10+10*(1-x)/(10*x+1))};
	\addlegendentry{$F_b$}
	
	
	\addplot [
	domain=0:1, 
	samples=100, 
	color=black,
	dashed
	]
	{10};
	
	
	%Here the blue parabloa is defined
	
	\end{axis}
	\end{tikzpicture}
	\caption{The revenue curve of distribution $F_b$ (dotted blue curve) used in the example, and $G_b$ (solid red curve) used for the analysis.}
	\label{fig:rev_curve_Gb}
\end{figure}


We now compute the revenue of the optimal mechanism for item $b$ with $\ell$ bidders. Instead of computing the revenue when $b$ is distributed according to $F_b$, we compute the revenue when $b$ is distributed according to $G_b(x)=1-\frac{1}{x-k+1}$.\footnote{One might wonder why we do not use $G_b$ instead of $F_b$ in the first place. The reason for this is that the benchmark only gives an upper bound for bounded distributions.} Since $G_b(x)\leq F_b(x)$ for every $x$, $G_b$ first-order stochastically dominates $F_b$. Since in a single item environment, the revenue of a dominating distribution is greater than the revenue of a dominated one (\cite{hart2015maximal}), this is enough in order to give an upper bound on the revenue of $F_b$. 
The revenue curve of $G_b$ is given in Figure \ref{fig:rev_curve_Gb}, where $R(1)= k$, $R(0)=1$, and $R(q)=1 + (k-1)q$ for $q\in (0,1)$. For a single bidder, the optimal mechanism sets a take-it-or-leave-it price of $k$ on the item, and gets an expected revenue of $k$. For two bidders, the optimal mechanism is $\VCG$ with monopoly reserves. Since the monopoly reserve is $k$, this is equivalent to just running $\VCG$. We compute the expected revenue of $\VCG$ the following way --- fix bidder $1$, and compute her expected payment. Bidder $2$'s value sets a random threshold for bidder $1$. If the quantile of bidder $2$'s value is $q$, then the bidder $1$'s expected payment is exactly the probability her value is above $v(q)$ \textit{times} $v(q)$. This is exactly $R(q)$. Therefore, the expected payment of bidder $1$ is exactly the area under the revenue curve, which is equal to $(k+1)/2$. By symmetry, bidder $2$'s expected payment is $(k+1)/2$ as well, and the expected revenue overall is $k+1$. Again, by submodularity of revenue, since the second bidder adds $1$ to the expected revenue, the expected revenue of $\VCG$ with $\ell$ bidders is at most $k+\ell-1$.

We get that the expected revenue obtained by running $\VCG$ on both items with $\ell$ bidders is at most $k+2\ell-1$. Therefore, $\ell$ has to be at least $\ln k /2 +1 = \Omega(\ln k)$ in order to cover the benchmark. Since $k$ can be arbitrary large, this benchmark is not suitable in providing any meaningful bound on the competition complexity for this market.

==> bk_additive.tex <==
NOT USED ANY MORE


\subsection{Single Additive Bidder}
With the new bound in hand, we show that we avoid the impossibility of Section \ref{sec:counterexample}.

\begin{theorem}
	Assuming regularity, VCG with $m$ more bidders $\geq \Rev$.
	%the results of Section \ref{sec:single-bidder-iid} hold without the i.i.d.~assumption.
\end{theorem}

\begin{proof}
	The proof is almost identical to the proof in Section \ref{sec:single-bidder-iid}.
	We state what changes in the proof of Proposition \ref{pro:work-horse} when we use the regions proposed in Section \ref{sec:quatile_regions}. Let $B_j$ be the event that $\forall j'\ne j: F_j(v_j)\ge F_{j'}(v_{j'})$ and let $\bar B_j$ be the event that $\exists j' : F_j(v_j)<F_{j'}(v_{j'})$.
	The upper bound on $\Rev$ becomes
	\begin{equation}
		\sum_j \sum_{v_j}\Pr[v_j] \left( \varphi_j(v_j)^+\cdot \Pr_{v_{-j}}[B_j] + v_j\cdot \Pr_{v_{-j}}[\bar B_j] \right).
		\label{eq:bench_noniid_single}
	\end{equation}
			
	$u$ is now a vector of i.i.d.~draws from $F_j$, whereas $v$ is a vector of independent draws from $F_1,F_2,\dots,F_m$. We couple $u$ and $v$ whenever  $F_{j'}(v_{j'})=F_{j}(u_{j'})$ for every coordinate $j'$.
	 %The coupling of $u$ and $v$ is the same, but the resulting value profiles $v,u$ after the quantiles have been drawn are different.
	 Still, bidder $j$ is allocated with precisely the probability that event $B_j$ occurs and its virtual value is positive (we are using here the monotonicity of $F_j$, i.e., that $u_j>u_{j'}$ for all $j'\ne j$ iff $F_j(v_j)=F_j(u_j)>F_j(u_{j'})=F_{j'}(v_{j'})$ for all $j'\ne j$). And in the second price auction, bidders other than $j$ win whenever event $\bar{B}_j$ occurs.
\end{proof}



==> duality.tex <==
\subsection{\cite{CDW16} Duality Framework}
In order to get Bulow-Klemperer type results, we adopt the duality framework presented by \cite{CDW16}. Consider the LP for maximizing revenue (Figure \ref{fig:LPRevenue}), where we add a type $\varnothing$ for the option of not participating in the auction (which implies $\pi_i(\varnothing)=\mathbf{0}$ and $p_i(\varnothing)= 0$). For each agent $i$, let $T_i^+=T_i\cup \{\varnothing\}$; this ensures that a BIC outcome will also imply a Bayesian IR outcome. \cite{CDW16} considered the following dual problem --- introduce a variable $\lambda_i(v,v')$ for each BIC constraint, and let $\mathcal{L}(\lambda,\pi, p)$ be the partial Lagrangian of the program in Figure \ref{fig:LPRevenue} by  Lagrangifying all BIC constraints. That is,

\begin{eqnarray}
\mathcal{L}(\lambda, \pi, p)&= &\sum_{i=1}^{n} \Big(\sum_{v_i \in T_i} f_{i}(v_{i})\cdot p_i(v_i)+\sum_{v_{i}\in T_{i}}\sum_{v_{i}'\in T_i^{+}} \lambda_{i}(v_{i},v_{i}')\cdot \Big(v_{i}\cdot\big(\pi(v_{i})-\pi({v_{i}'})\big)-\big(p_{i}(v_{i})-p_{i}(v_{i}')\big)\Big)\Big)\nonumber\\
&= & \sum_{i=1}^n \sum_{v_{i}\in T_{i}} p_{i}(v_{i})\Big(f_{i}(v_{i})+\sum_{v_{i}'\in T_{i}} \lambda_{i}(v_{i}',v_{i})-\sum_{v_{i}'\in T_{i}^{+}} \lambda_{i}(v_{i},v_{i}')\Big)\nonumber\\
& &+\sum_{i=1}^n\sum_{v_{i}\in T_{i}}\pi_{i}(v_{i}) \Big(\sum_{v_{i}'\in T_{i}^{+}}v_i \cdot \lambda_{i}(v_{i},v_{i}')-\sum_{t'_{i}\in T_{i}}v_{i}'\cdot \lambda_{i}(v_{i}',v_{i})\Big) \label{eq:lagrangian} %\\ ~~~~~~~~~~~~({\pi}_i(\varnothing)=\textbf{0},\ p_{i}(\varnothing)=0)\
\end{eqnarray}
% &~~~~~~~~~~~~({\pi}_i(\varnothing)=\textbf{0},\ p_{i}(\varnothing)=0)\stepcounter{equation}\tag{\theequation} \label{eq:dual lagrangian}
The partially Lagrangified dual of the revenue maximization LP is given if Figure \ref{fig:Lagrangian}.

\begin{figure}[ht]
	\colorbox{MyGray}{
		\begin{minipage}{\textwidth} {
			\noindent\textbf{Variables:}
			\begin{itemize}
				\item $p_i(v_i)$, for all bidders $i$ and types $v_i \in T_i$, denoting the expected price paid by bidder $i$ when reporting type $v_i$ over the randomness of the mechanism and the other bidders' types.
				\item $\pi_{ij}(v_i)$, for all bidders $i$, items $j$, and types $v_i \in T_i$, denoting the probability that bidder $i$ receives item $j$ when reporting type $v_i$ over the randomness of the mechanism and the other bidders' types.
			\end{itemize}
			\textbf{Constraints:}
				\begin{itemize}
					\item ${\pi}_i(v_i) \cdot v_i - p_i(v_i) \geq {\pi}_i(v'_i)\cdot v_i - p_i(v'_i) $, for all bidders $i$, and types $v_i \in T_i, v'_i \in T_i^+$, guaranteeing that the reduced form mechanism $({\pi},{p})$ is BIC and Bayesian IR.
					%\item ${\pi}_i(t_i) \cdot t_i - p_i(t_i) \geq 0$, for all bidders $i$, and types $t_i \in T_i$, guaranteeing that the reduced form mechanism $({\pi},{p})$ is individually rational.
					\item ${\pi} \in \polytope$, guaranteeing ${\pi}$ is feasible.
				\end{itemize}
			\textbf{Objective:}
			\begin{itemize}
				\item $\max \sum_{i=1}^{n} \sum_{t_i \in T_i} f_{i}(v_{i})\cdot p_i(v_i)$, the expected revenue.\\
			\end{itemize}							
		}\end{minipage}
	}
	\caption{A Linear Program (LP) for Revenue Optimization.}
	\label{fig:LPRevenue}
\end{figure}



\begin{figure}[ht!]
\colorbox{MyGray}{
\begin{minipage}{\textwidth} {
		\noindent\textbf{Variables:}
		\begin{itemize}
			\item $\lambda_i(v_{i},v_{i}')$ for all $i,v_{i}\in T_{i},v_{i}' \in T_i^{+}$, the Lagrangian multipliers for Bayesian IC constraints.
		\end{itemize}
		\textbf{Constraints:}
		\begin{itemize}
			\item $\lambda_i(v_{i},v_{i}')\geq 0$ for all $i,v_{i}\in T_{i},v_{i}' \in T_i^{+}$, guaranteeing that the Lagrangian multipliers are non-negative. 
		\end{itemize}
		\textbf{Objective:}
		\begin{itemize}
			\item $\min_{\lambda}\max_{\pi\in\polytope, p} \mathcal{L}(\lambda, \pi, p)$.\\
		\end{itemize}}
	\end{minipage}}
	\caption{Partial Lagrangian of the Revenue Maximization LP.}
	\label{fig:Lagrangian}
\end{figure}

Strong duality implies that every upper bound we have on the value of the dual program is also an upper bound on the optimal revenue the seller can make. \cite{CDW16} showed that by choosing the dual variables carefully, they can give meaningful bounds for the value of the dual, which are useful in order to proof approximation results. In particular, consider the following flow network:
\begin{itemize}
	\item Nodes: A super source $s$ and a super sink $\varnothing$, along with a node $v_{i}$ for every type $v_{i}\in T_{i}$. 
	\item Flow from $s$ to $v_{i}$ of weight $f_i(v_{i})$, for all $v_{i}\in T_{i}$.
	\item Flow from $v_i$ to $v'_i$ of weight $\lambda_i(v_i,v'_i)$ for all $v_i\in T$, and $v'_i\in T_{i}^{+}$ (including the sink).
\end{itemize}

They showed that in order for the dual variables to be useful, the above network must be a valid flow network.
\begin{lemma}[\cite{CDW16}]\label{lem:useful_dual}
	The value of the dual program in Figure \ref{fig:Lagrangian} is finite if and only if the flow network defined by the dual satisfies flow conservation; that is, for any vertex $v_i\in T_i$,
	\begin{eqnarray}
		f_i(v_i)+\sum_{v'_i\in T_i} \lambda(v'_i,v_i)=\sum_{v'_i\in T_i^+} \lambda(v_i,v'_i). \label{eq:conserv}
	\end{eqnarray}
\end{lemma}
It is easy to see that if Eq. $(\ref{eq:conserv})$ does not hold for some type $v_i$ of some agent $i$, then it is possible to set $p_i(v_i)$ either to $\infty$ or $-\infty$, and consequently, the value of $\mathcal{L}(\lambda, \pi, p)$ (Eq. $(\ref{eq:lagrangian})$) and the dual would be unbounded.

For their multi-dimentional \cite{CDW16} defined a virtual valuation as follows.
\begin{definition}[Virtual Value Function]
	Given the dual variables $\lambda$, the virtual valuation function $\Phi_i(\cdot)$ is defined to be
	$$\Phi_{i}(v_{i})=v_{i}-{1\over f_{i}(v_{i})}\sum_{v_{i}'\in T_{i}} \lambda_{i}(v_{i}',v_{i})(v_{i}'-v_{i}).$$
\end{definition}
In the spirit of \cite{myerson1981optimal}, \cite{CDW16} showed that the revenue of a truthful mechanism is no more than the expected virtual value of the mechanism.
\begin{theorem}[\cite{CDW16} Revenue $\leq$ Virtual Welfare]\label{thm:revenue less than virtual welfare}
	Let $\lambda$ be a valid flow (which satisfies Eq. $(\ref{eq:conserv})$ for any $i$ and $v_i\in T_i$), and $M = (\pi,p)$ any BIC mechanism. Then the revenue of $M$ is $\leq$  the virtual welfare of $\pi$ w.r.t. the virtual value function $\Phi(\cdot)$ corresponding to $\lambda$. That is:
	$$\sum_{i=1}^{n} \sum_{v_i \in T_i} f_{i}(v_{i})\cdot p_i(v_i)\leq \sum_{i=1}^{n} \sum_{v_{i}\in T_{i}} f_{i}(v_{i})\cdot \pi_{i}(v_{i})\cdot\Phi_{i}(v_{i}).$$
	%Furthermore, let $\lambda^{*}$ be the optimal dual variables and $M^{*}=(\pi^{*},p^{*})$ be the revenue optimal BIC mechanism, then the expected virtual welfare with respect to $\Phi^{*}$ (induced by $\lambda^{*}$) under  $\pi^{*}$ equals the expected revenue of $M^{*}${, and $$\pi^* \in \arg\max_{\pi \in \polytope}\left\{\sum_{i=1}^n \sum_{t_i \in T_i} f_i(t_i) \pi_i(t_i) \Phi^*_i(t_i)\right\}.$$
\end{theorem}

\subsubsection{Region-based Flow}
We now present a region based flow that will be used to get Bulow-Klemperer type results. This presentation is slightly more general than the one used in \cite{CDW16}, and the regions presented are general \textit{\textbf{upward-closed regions}}, meaning that if a for some $v_i=(v_{ij}, v_{i-j})\in T_i$ and $v_{-i}\in T_{-i}$, $v_i$ is in region $R_j({v_{-i}})$, then for all $v'_{ij}\geq v_{ij}$ such that $v'_i=(v'_{ij}, v_{i-j})\in T_i$, $v'_i$ is also in $R_j({v_{-i}})$. The intuition behind the region-based flow is as follows --- a naive upper bound on the expected revenue is the expected welfare of the sampled valuations. This upper bound is overly optimistic\footnote{Consider the equal revenue distribution $F(x)=1-1/x$, where the expected optimal revenue is 1, while the expected welfare is infinite.}. To overcome this, \cite{CDW16} used the region-based flow as following --- for some value $v_i\in R_j({v_{-i}})$, the flow based benchmark keeps the values $v_{ik}$ for all $k\neq j$, and truncates $v_{ij}$ to $\varphi(v_{ij}) < v_{ij}$, where $\varphi(v_{ij})$ is Myerson's virtual value function. \cite{CDW16} showed that by choosing the regions according to item that grants the agent the highest utility, suffices in order to design approximately optimal simple mechanisms. As we show in XXX, this is not sufficient when trying to prove Bulow-Klemperer type results. We therefore modify regions to be based according to the item of the highest quantile\footnote{We use the convention where the quantile of $v_{ij}$ is $q_{ij}(v_{ij})=F_{ij}(v_{ij})$.} of the agent.

We now describe the region-based flow. Given valuation profile $v_{-i}$ of all bidders besides $i$, we partition the type space $T_i$ into $m+1$ upward-closed regions $R_0({v_{-i}}),R_1({v_{-i}}),\ldots, R_m({v_{-i}})$. We first define a flow $\lambda_i^{v_{-i}}$ for the possible valuation types of agent $i$, which depends on $v_{-i}$.
\begin{itemize}
	\item For every type $v_i$ in region $R_0({v_{-i}})$, direct all incoming flow to the sink $\varnothing$.
	\item For every type $v_i=(v_{ij},v_{i-j})$ in region $R_j({v_{-i}})$ direct flow to $v'_i=(v'_{ij},v_{i-j})$, where $v'_{ij}$ is the largest value in the support of $F_{ij}$ smaller than $v_{ij}$, if exists. Otherwise, direct all flow to $\varnothing$. 
\end{itemize}
Let $\Phi_i^{v_{-i}}(\cdot)$ be the corresponding virtual value to the flow depicted above, a simple adaptation of Claims 1 and 2 in \cite{CDW16} to general upwards closed regions yields the following properties for $\Phi_i^{v_{-i}}(\cdot)$.
\begin{lemma}\label{lem:virtual_sup}
	Let $v_i\in T_i$ and $v_{-i}\in T_{-i}$ be some valuation profile for which $v_i\in R_j({v_{-i}})$ for some $j\in \{0,\ldots,m\}$. Then $\Phi_{ik}^{v_{-i}}(v_i)=v_{ik}$ if $k\neq j$ and $\Phi_{ij}^{v_{-i}}(v_i)=\varphi_{ij}(v_{ij})$ (if $j\neq 0$) where $\varphi_{ij}(\cdot)$ is Myerson's virtual valuation function for distribution $F_{ij}$.
\end{lemma}
\Q{Should we discuss the irregular case here?}
A proof for this lemma is given in Appendix XXX. Since we fix the flow of agent $i$ in advance, regardless of the agent's report, we average the flow $\lambda_i$ across the different valuation profiles $v_{-i}\in T_{-i}$ the agents might take.  
\begin{definition}[Flow]
	Given $m+1$ upward closed regions $R_0(\cdot),R_1(\cdot),\ldots,R_m(\cdot)$, The flow for bidder $i$ is $\lambda_i=\sum_{v_{-i}\in T_{-i}}f_{-i}(v_{-i})\lambda_i^{v_{-i}}$, and the corresponding virtual value function of agent $i$ for flow $\lambda_i$ is $\Phi_i(\cdot)=\sum_{v_{-i}\in T_{-i}} f_{-i}(v_{-i})\Phi_i^{v_{-i}}(\cdot).$
\end{definition}
Applying Lemma \ref{lem:virtual_sup}, we get the following.
\begin{lemma}\label{lem:virtual}
	For all $i, j$ and $v_{i}\in T_i$, $$\Phi_{ij}(v_i)=\varphi_{ij}(v_{ij})\cdot\Pr_{v_{-i}\sim F_{-i}}\left[v_i\in R_j(v_{-i})\right]+v_{ij}\cdot\Pr_{v_{-i}\sim F_{-i}}\left[v_i\notin R_j(v_{-i})\right].$$
\end{lemma}
Using the region-based flow, we get the following upper bound on the revenue of any  BIC mechanism.
\begin{theorem}
	For any set of upward-closed regions $R_0,\ldots, R_m$, the optimal revenue a seller can obtain by a BIC mechanism is upper bounded by 
	\begin{eqnarray} 
		\max_{\pi\in \polytope}\sum_i \sum_{v_i\in T_i}\sum_j f_i(v_i) \cdot \pi_{ij}(v_i) \left(\varphi_{ij}(v_{ij})\cdot\Pr_{v_{-i}\sim F_{-i}}\left[v_i\in R_j(v_{-i})\right]+v_{ij}\cdot\Pr_{v_{-i}\sim F_{-i}}\left[v_i\notin R_j(v_{-i})\right]\right).\label{eq:rev_upper_bound}
	\end{eqnarray}
	%Let $M$ be a BIC mechanism with $(\pi, p)$ as its reduced form. The expected revenue of $M$ 
\end{theorem}
\begin{proof}
	A direct corollary of Theorem \ref{thm:revenue less than virtual welfare} and Lemma \ref{lem:virtual}.
\end{proof}

\subsubsection{Regions Used in \cite{CDW16}, Single Additive Bidder Case}
We now present the single additive bidder case bound used in \cite{CDW16}. Even for this case, the bound they use is too high in order to get a meaningful bound on the number of bidders that one needs to add in order to get a higher revenue using a VCG mechanism. This is demonstrated in Section \ref{sec:counterexample}. 
Since we deal with only a single bidder, the bound of $(\ref{eq:rev_upper_bound})$ simplifies to 
\begin{eqnarray*}
\Rev\leq \max_{\pi} \sum_{v\in T}\sum_j f(v) \cdot \pi_{j}(v) \left(\varphi_j(v_{j})\cdot\mathbb{I}\left[v\in R_j \right]+v_{j}\cdot \mathbb{I}\left[v\notin R_j\right]\right).
\end{eqnarray*}
For a single additive bidder, there are no feasibility constraints across items. Also, for the max to be achieved, for a valuation $v\in R_j$ where $\varphi_j(v_j)<0$, $\pi_j(v)$ has to be equal to $0$. Therefore, the upper bound can be re-written as
\begin{eqnarray}
\Rev&\leq& \sum_{v\in T}\sum_j f(v)  \left(\varphi_j(v_{j})^+\cdot\mathbb{I}\left[v\in R_j \right]+v_{j}\cdot \mathbb{I}\left[v\notin R_j\right]\right)\nonumber\\
& = & \mathbb{E}_{v\sim F} \Big[ \sum_j\left(\ \varphi_j(v_j)^+ \cdot \mathbb{I}[v\in R_j ] + v_j \cdot \mathbb{I}[v\notin R_j ]\ \right) \Big]\nonumber\\ 
&= &\sum_j \sum_{v_j}\Pr[v_j] \left( \varphi_j(v_j)^+\cdot \Pr_{v_{-j}}[v\in R_j ] + v_j\cdot \Pr_{v_{-j}}[v\notin R_j ] \right).\label{eq:bench_single_bidder}
\end{eqnarray}

Up until now, we gave an upper bound that for generic upward-closed feasibility. \cite{CDW16} defined region $R_j$ to contain all valuations $v=(v_1,\ldots,v_m)$ for which $v_j\geq v_k$ for every $j'\neq j$ (breaking ties lexicographically). Therefore, they get the following bound:
\begin{eqnarray}
\Rev\leq \sum_j \sum_{v_j}\Pr[v_j] \left( \varphi_j(v_j)^+\cdot \Pr_{v_{-j}}[\forall j'\neq j : v_j\geq v'_j ] + v_j\cdot \Pr_{v_{-j}}[\exists j': v_j< v'_j ] \right).\label{eq:bench_single_cdw}
\end{eqnarray}

==> dualityApp.tex <==
Consider the revenue maximization linear program defined in Figure \ref{fig:LPRevenue}.
As in  \cite{CDW16}, the extra type $\varnothing$ represents a non-participating agent. 
Let $T_i^+=T_i\cup \{\varnothing\}$\footnote{\ofnote{This ensures that the linear program accounts for both BIC and BIR mechanisms.}}.
By introducing a dual $\lambda_i(v,v')$ for each BIC constraint, we get the following partial Lagrangian $\mathcal{L}(\lambda,\pi, p)$ (the partially Lagrangified dual is given if Figure \ref{fig:Lagrangian}.):

\begin{eqnarray*}
\mathcal{L}(\lambda, \pi, p) %& = &\sum_{i=1}^{n} \Big(\sum_{v_i \in T_i} f_{i}(v_{i})\cdot p_i(v_i)+\sum_{v_{i}\in T_{i}}\sum_{v_{i}'\in T_i^{+}} \lambda_{i}(v_{i},v_{i}')\cdot \Big(v_{i}\cdot\big(\pi(v_{i})-\pi({v_{i}'})\big)-\big(p_{i}(v_{i})-p_{i}(v_{i}')\big)\Big)\Big)\nonumber\\
&= & \sum_{i=1}^n \sum_{v_{i}\in T_{i}} p_{i}(v_{i})\Big(f_{i}(v_{i})+\sum_{v_{i}'\in T_{i}} \lambda_{i}(v_{i}',v_{i})-\sum_{v_{i}'\in T_{i}^{+}} \lambda_{i}(v_{i},v_{i}')\Big)\nonumber\\
& &+\sum_{i=1}^n\sum_{v_{i}\in T_{i}}\pi_{i}(v_{i}) \Big(\sum_{v_{i}'\in T_{i}^{+}}v_i \cdot \lambda_{i}(v_{i},v_{i}')-\sum_{v'_{i}\in T_{i}}v_{i}'\cdot \lambda_{i}(v_{i}',v_{i})\Big) \label{eq:lagrangian} %\\ ~~~~~~~~~~~~({\pi}_i(\varnothing)=\textbf{0},\ p_{i}(\varnothing)=0)\
\end{eqnarray*}
% &~~~~~~~~~~~~({\pi}_i(\varnothing)=\textbf{0},\ p_{i}(\varnothing)=0)\stepcounter{equation}\tag{\theequation} \label{eq:dual lagrangian}

\begin{figure}[ht]
	\colorbox{MyGray}{
		\begin{minipage}{\textwidth} {
				\noindent\textbf{Variables:}
				\begin{itemize}
					\item $p_i(v_i)$, for all bidders $i$ and types $v_i \in T_i$, denoting the expected price paid by bidder $i$ when reporting type $v_i$ over the randomness of the mechanism and the other bidders' types.
					\item $\pi_{ij}(v_i)$, for all bidders $i$, items $j$, and types $v_i \in T_i$, denoting the probability that bidder $i$ receives item $j$ when reporting type $v_i$ over the randomness of the mechanism and the other bidders' types. Denote by $\pi_i(v_i)$ the vector $(\pi_{i1}(v_i), \dots, \pi_{im}(v_i))$.
				\end{itemize}
				\textbf{Constraints:}
				\begin{itemize}
					\item ${\pi}_i(v_i) \cdot v_i - p_i(v_i) \geq {\pi}_i(v'_i)\cdot v_i - p_i(v'_i) $, for all bidders $i$, and types $v_i \in T_i, v'_i \in T_i^+$, guaranteeing that the reduced form mechanism $({\pi},{p})$ is BIC and Bayesian IR.
					%\item ${\pi}_i(t_i) \cdot t_i - p_i(t_i) \geq 0$, for all bidders $i$, and types $t_i \in T_i$, guaranteeing that the reduced form mechanism $({\pi},{p})$ is individually rational.
					\item ${\pi} \in \polytope$, guaranteeing ${\pi}$ is feasible.
				\end{itemize}
				\textbf{Objective:}
				\begin{itemize}
					\item $\max \sum_{i=1}^{n} \sum_{v_i \in T_i} f_{i}(v_{i})\cdot p_i(v_i)$, the expected revenue.\\
				\end{itemize}							
			}\end{minipage}
		}
		\caption{A Linear Program (LP) for Additive Revenue Optimization.}
		\label{fig:LPRevenue}
	\end{figure}
	
	
	
	\begin{figure}[ht!]
		\colorbox{MyGray}{
			\begin{minipage}{\textwidth} {
					\noindent\textbf{Variables:}
					\begin{itemize}
						\item $\lambda_i(v_{i},v_{i}')$ for all $i,v_{i}\in T_{i},v_{i}' \in T_i^{+}$, the Lagrangian multipliers for Bayesian IC constraints.
					\end{itemize}
					\textbf{Constraints:}
					\begin{itemize}
						\item $\lambda_i(v_{i},v_{i}')\geq 0$ for all $i,v_{i}\in T_{i},v_{i}' \in T_i^{+}$, guaranteeing that the Lagrangian multipliers are non-negative.
					\end{itemize}
					\textbf{Objective:}
					\begin{itemize}
						\item $\min_{\lambda}\max_{\pi\in\polytope, p} \mathcal{L}(\lambda, \pi, p)$.\\
					\end{itemize}}
				\end{minipage}}
				\caption{Partial Lagrangian of the Revenue Maximization LP.}
				\label{fig:Lagrangian}
			\end{figure}
			
			Strong duality implies that every upper bound we have on the value of the dual program is also an upper bound on the optimal revenue the seller can make. \cite{CDW16} showed that by choosing the dual variables carefully, they can give meaningful bounds for the value of the dual, which are useful in order to prove approximation results. In particular, consider the following flow network:
			\begin{itemize}
				\item Nodes: A super source $s$ and a super sink $\varnothing$, along with a node $v_{i}$ for every type $v_{i}\in T_{i}$.
				\item Flow from $s$ to $v_{i}$ of weight $f_i(v_{i})$, for all $v_{i}\in T_{i}$.
				\item Flow from $v_i$ to $v'_i$ of weight $\lambda_i(v_i,v'_i)$ for all $v_i\in T$, and $v'_i\in T_{i}^{+}$ (including the sink).
			\end{itemize}
			
			They showed that in order for the dual variables to be useful, the above network must be a valid flow network.
			\begin{lemma}[\cite{CDW16}]\label{lem:useful_dual}
				The value of the dual program in Figure \ref{fig:Lagrangian} is finite if and only if the flow network defined by the dual satisfies flow conservation; that is, for any vertex $v_i\in T_i$,
				\begin{eqnarray}
				f_i(v_i)+\sum_{v'_i\in T_i} \lambda(v'_i,v_i)=\sum_{v'_i\in T_i^+} \lambda(v_i,v'_i). \label{eq:conserv}
				\end{eqnarray}
			\end{lemma}

%			It is easy to see that if Eq. $(\ref{eq:conserv})$ does not hold for some type $v_i$ of some agent $i$, then it is possible to set $p_i(v_i)$ either to $\infty$ or $-\infty$, and consequently, the value of $\mathcal{L}(\lambda, \pi, p)$ (Eq. $(\ref{eq:lagrangian})$) and the dual would be unbounded.
%			
			For their multi-dimensional setting, \cite{CDW16} defined a virtual valuation as follows:
			\begin{definition}[Virtual Value Function]
				Given the dual variables $\lambda$, the virtual valuation function $\Phi_i(\cdot)$ is defined to be
				$$\Phi_{i}(v_{i})=v_{i}-{1\over f_{i}(v_{i})}\sum_{v_{i}'\in T_{i}} \lambda_{i}(v_{i}',v_{i})(v_{i}'-v_{i}).$$
			\end{definition}
			
			%In the spirit of \cite{myerson1981optimal},
\cite{CDW16} showed that the revenue of a truthful mechanism is no more than the expected virtual value of the mechanism. This is cast in the following theorem.

==> mult_constraint_add_missing.tex <==

	
	~
	
\noindent\textbf{Proof of Claim \ref{clm:single_allocated}:} 
	We argue that if $j$ is allocated to an agent $i\in \bar{A}$, the allocation of all other items in $\OPT$ is identical to their allocation in $\OPT_{-j}$, and so precisely one bidder in $\bar{A}$ is allocated by VCG, as required. Items are allocated as in $\OPT_{-j}$ due to the downward-closedness of the constraints on the bidders' additive valuations; we now show that assuming otherwise leads to a contradiction: Consider the allocation $\OPT_{-j}$, and assume for contradiction that after a bidder $i\in\bar{A}$ is allocated item $j$, to get to allocation $\OPT$ we need to perform additional reallocations of items. By the consistency of VCG's tie breaking rule this means that we need additional reallocations to get to the optimal welfare. Because valuations are additive subject to downward-closed constraints, if we can increase the total welfare by item reallocations when bidder $i$ has item $j$, we can get the same increase in welfare by these reallocations when bidder $i$ does not have item $j$. This contradicts the optimality of $\OPT_{-j}$, and completes the proof of the claim.\qed

~




==> newBound.tex <==
\textbf{Proof of Theorem~\ref{thm:new_bound}}
Notice that in Equation~(\ref{eq:rev_upper_bound}), since there are no feasibility constraints, $\pi_{ij}(\cdot)$ can allocate each item to the non-negative,  maximizing, virtual value. Therefore:
\begin{eqnarray*}
	\Rev &\leq & \max_{\pi} \mathbb{E}_{\vals \sim F^n}\left[\sum_{i=1}^n \sum_{j=1}^m \pi_{ij}(v_i) \bigg(\varphi_{ij}(v_{ij})^+\cdot\mathbb{I}_{v_i\in R_j}\ + \ v_{ij}\cdot\mathbb{I}_{v_i\notin R_j}\bigg)\right] \\
	&= & \mathbb{E}_{\vals \sim F^n}\left[ \sum_{j=1}^m \max_{i\in [n]} \bigg(\varphi_{ij}(v_{ij})^+\cdot\mathbb{I}_{v_i\in R_j}\ + \ v_{ij}\cdot\mathbb{I}_{v_i\notin R_j}\bigg)\right] \\
	&= & \sum_{j=1}^m \mathbb{E}_{\vals \sim F^n}\left[ \max_{i\in [n]} \bigg(\varphi_{ij}(v_{ij})^+\cdot\mathbb{I}_{v_i\in R_j}\ + \ v_{ij}\cdot\mathbb{I}_{v_i\notin R_j}\bigg)\right].
\end{eqnarray*}



==> new_flow.tex <==
NOT USED ANY MORE

\subsubsection{Example where Previous Benchmark Fails} \label{sec:counterexample}

In our example with $2$ items, one with an equal revenue distribution capped at $k$, and the other with distribution $F(x)=1-\frac{k\epsilon}{x-(1-\epsilon)k}$ on the support $(k,\infty)$ \itcomment{Explain the intuition behind this distribution, why adding bidders raises the revenue by a really small amount.}, the revenue benchmark in \eqref{eq:bench2} is $k+\log k$, whereas the benchmark according to Proposition \ref{pro:new-bench} is $k+2$. \itcomment{Verify this.} The tighter benchmark allows us to show that $\sum_j \Mye_m(j)\ge \Rev$.

\subsubsection{Quantile Based Regions}\label{sec:quatile_regions}
As previously discussed, the proof of the case where the items are sampled from the same distribution does not extend when the items are not i.i.d. The reason is that the probability of the $j$th sample to be the highest one (that is, the probability that $v\in R_j$) is not same as the probability of agent $j$ to have the highest value for item $j$, since the samples of the agents' values for item $j$ \textbf{are} i.i.d. The intuition behind the regions we use is that we want to mimic the buyers' i.i.d. samples, even if the items themselves are not i.i.d.

We change the regions the following way --- we define $$R_j=\{v : \forall j'\ne j \ \  F_j(v_j) > F_{j'}(v_{j'}) \},$$
that is, for each bidder, region $j$ is defined as the region where the agent value is of the highest quantile according to the items' distributions. Now, one may notice that the probability that some valuation $v$ is in $R_j$ equals exactly the probability that in $m$ i.i.d. samples from $F_j$, the $j$th sample is the highest.

We rewrite $(\ref{eq:rev_upper_bound})$ for additive bidders, meaning that there are no feasibility constraints across items, but an item cannot  be allocated more then once. Furthermore, we assume all bidders are drawn i.i.d. from a product distribution $F=F_1\times\ldots\times F_m$, and therefore, $\varphi_{ij}=\varphi_j$ for every $i$:
\begin{eqnarray}
	\Rev & \leq & \max_{\pi}\E_{\vals\sim F^n}\left[\sum_{i=1}^n\sum_{j=1}^m \pi_{ij}(v_i)\bigg(\varphi_{j}(v_{ij})^+\cdot\mathbb{I}_{v_i\in R_j} \ + \ v_{ij}\cdot\mathbb{I}_{v_i\notin R_j}\bigg)\right]\nonumber\\
	& = & \E_{\vals\sim F^n}\left[\sum_{j=1}^m\max_{i\in [n]}\bigg(\varphi_{j}(v_{ij})^+\cdot\mathbb{I}_{v_i\in R_j} \ + \ v_{ij}\cdot\mathbb{I}_{v_i\notin R_j}\bigg)\right] \nonumber\\
	& = & \sum_{j=1}^m\E_{\vals\sim F^n}\left[\max_{i\in [n]}\bigg(\varphi_{j}(v_{ij})^+\cdot\mathbb{I}_{v_i\in R_j} \ + \ v_{ij}\cdot\mathbb{I}_{v_i\notin R_j}\bigg)\right].\label{eq:multiple_new_flow}
\end{eqnarray}
\begin{comment}
\subsection{Single Additive Bidder}

Let

\begin{proposition}
	\label{pro:new-bench}
	%Assume regularity.
	Let $B_j$ be the event that $\forall j'\ne j: F_j(v_j)\ge F_{j'}(v_{j'})$ and let $\bar B_j$ be the event that $\exists j' : F_j(v_j)<F_{j'}(v_{j'})$.
	\begin{equation}
	\Rev \le \sum_j \sum_{v_j}\Pr[v_j]\cdot \left( \varphi_j(v_j)^+\cdot \Pr_{v_{-j}}[B_j] + v_j\cdot \Pr_{v_{-j}}[\bar B_j] \right).
\label{eq:bench2}
	\end{equation}
\end{proposition}
	
\begin{proof}
	By defining the regions to be $R_j=\{v : \forall j'\ne j \ \  F_j(v_j)\ge F_{j'}(v_{j'}) \}$ and applying Eq. $(\ref{eq:bench_single_bidder})$.
\end{proof}

\subsection{Multiple Additive Bidders}
		
Assume regularity. Let $B_{ij}$ be the event that $\forall k\ne j: F_j(v_{ij}) > F_k(v_{ik})$. Let $\bar{B}_{ij}$ be the event that $\exists k\ne j: F_j(v_{ij}) < F_k(v_{ik})$. Let $x=\vec{x}$ be an $nm$-vector.
		
\begin{eqnarray}
	\Rev &\le& \max_{\text{feasible } x}\E_v[\sum_{ij}\Phi_{ij}(v_i)x_{ij}(v)]\nonumber\\
	&=& \max_{\text{feasible } x}\E_v[x_{ij}(v) \sum_{ij}\left(\varphi_{j}(v_{ij})^+I(B_{ij})+ v_{ij}I(\bar{B}_{ij})\right)]\nonumber\\
	&=& \E_v[\sum_j \max_i\{\varphi_{j}(v_{ij})^+I(B_{ij})+ v_{ij}I(\bar{B}_{ij})\}]\nonumber\\
	&=& \sum_j \E_v[\max_i\{\varphi_{j}(v_{ij})^+I(B_{ij})+ v_{ij}I(\bar{B}_{ij})\}].\label{eq:new-bench-multi}
\end{eqnarray}
\end{comment} 
